Reversing the cycle: self-supervised deep stereo through enhanced monocular distillation

In many fields, self-supervised learning solutions are rapidly evolving and filling the gap with supervised approaches. This fact occurs for depth estimation based on either monocular or stereo, with the latter often providing a valid source of self-supervision for the former. In contrast, to soften typical stereo artefacts, we propose a novel self-supervised paradigm reversing the link between the two. Purposely, in order to train deep stereo networks, we distill knowledge through a monocular completion network. This architecture exploits single-image clues and few sparse points, sourced by traditional stereo algorithms, to estimate dense yet accurate disparity maps by means of a consensus mechanism over multiple estimations. We thoroughly evaluate with popular stereo datasets the impact of different supervisory signals showing how stereo networks trained with our paradigm outperform existing self-supervised frameworks. Finally, our proposal achieves notable generalization capabilities dealing with domain shift issues. Code available at https://github.com/FilippoAleotti/Reversing

==> figures/middlebury_qualitatives.tex <==
\begin{figure}[t]
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccccc}
        \small{Reference} & \small{GT} & \small{\textcolor{blue}{Wang}} \cite{wang2019unos} & \small{\textcolor{blue}{Lai}} \cite{lai2019bridging} & \small{\textcolor{blue}{\textbf{Ours}}} \cite{Chang_2018_CVPR} & \small{\textcolor{red}{Zhang }} \cite{Zhang2019GANet} \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-gt.png} &        
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-ganet.png}
        \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-gt.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-ganet.png}
        \\
    \end{tabular}
    \caption{\textbf{Examples of generalization}. The first row shows disparity maps obtained from a stereo pair from the Middlebury v3 dataset, while second from ETH3D. Methods in \textcolor{blue}{\textbf{blue}} represent self-supervised stereo networks, while in \textcolor{red}{\textbf{red}} are supervised with ground-truth. }
    \label{fig:qualitatives_mid}
\end{figure}

%%%%%%%%%%%%%%%%
%% SUPPLEMENTARY
%%%%%%%%%%%%%%%%
\iffalse
\begin{figure}
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccccc}
        \small{Reference} & \small{GT} & \small{\textcolor{blue}{Wang}} \cite{wang2019unos} & \small{\textcolor{blue}{Lai}} \cite{lai2019bridging} & \small{\textcolor{blue}{\textbf{Ours}}} \cite{Chang_2018_CVPR} & \small{\textcolor{red}{Zhang }} \cite{Zhang2019GANet} \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Vintage.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Vintage-gt.png} &        
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Vintage-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Vintage-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Vintage-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Vintage-ganet.png} 
        \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-gt.png} &        
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Jadeplant-ganet.png}
        \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Pipes.png} & 
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Pipes-gt.png} &         
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Pipes-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Pipes-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Pipes-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/middlebury/Pipes-ganet.png}
        \\
    \end{tabular}
    \caption{\textbf{Examples of generalization}. }
    \label{fig:qualitatives_mid}
\end{figure}



\begin{figure}
    \centering
    \renewcommand{\tabcolsep}{0.5pt}
    \begin{tabular}{cccccc}
        \small{Reference} & \small{GT} & \small{\textcolor{blue}{Wang}} \cite{wang2019unos} & \small{\textcolor{blue}{Lai}} \cite{lai2019bridging} & \small{\textcolor{blue}{\textbf{Ours}}} \cite{Chang_2018_CVPR} & \small{\textcolor{red}{Zhang }} \cite{Zhang2019GANet} \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_3s.png} & 
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_3s-gt.png} & 
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_3s-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_3s-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_3s-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_3s-ganet.png} 
        \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_1s.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_1s-gt.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_1s-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_1s-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_1s-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/electro_1s-ganet.png}  
        \\
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-gt.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-unos.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-bridging.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-psm-ours.png} &
        \includegraphics[width=0.16\textwidth]{images/qualitatives/eth/playground_2l-ganet.png}  
    \end{tabular}
     \caption{\textbf{Qualitative on ETH3D}. Methods in \textcolor{blue}{\textbf{blue}} are self-supervised, while in \textcolor{red}{\textbf{red}} are supervised with ground-truth.}
    \label{fig:qualitatives_eth}
\end{figure}
\fi

